Investigating Layer Importance in Large Language Models

Large language models (LLMs) have gained increasing attention due to their prominent ability to understand and process texts. Nevertheless, LLMs largely remain opaque. The lack of understanding of LLMs has obstructed the deployment in safety-critical scenarios and hindered the development of better models. In this study, we advance the understanding of LLM by investigating the significance of individual layers in LLMs. We propose an efficient sampling method to faithfully evaluate the importance of layers using Shapley values, a widely used explanation framework in feature attribution and data valuation. In addition, we conduct layer ablation experiments to assess the performance degradation resulting from the exclusion of specific layers. Our findings reveal the existence of cornerstone layers, wherein certain early layers can exhibit a dominant contribution over others. Removing one cornerstone layer leads to a drastic collapse of the model performance, often reducing it to random guessing. Conversely, removing non-cornerstone layers results in only marginal performance changes. This study identifies cornerstone layers in LLMs and underscores their critical role for future research.

==> note.tex <==
Investigate task-specific layer importance for large language models

define stand-alone layer importance

show two main results
1. MLP is in general more important
2. show a contrastive behavior: for QA tasks, not all layers are important. For text generation tasks, all layers exhibit adequate importance

Hypothesis: model knows the answer during early layer processing. 

discuss limitation


existence of decision layer in large language models

main finding, for many QA tasks, there exists a decision layer, where removing this single layer causes the model to perform randomly on the target task. Intriguingly, the decision layer is usually in the earlier layer, and is a MLP layer. 

Update 06062024

Use shapley value to evaluate the importance of layers. 
Two restriction:
1. dont remove too much layers (thresholding sampling)
2. constrained to remove consecutive layers (assume neibouring layers works together)

